A transitivity result for ad-nilpotent ideals in type A

The paper considers subspaces of the strictly upper triangular matrices, which are stable under Lie bracket with any upper triangular matrix. These subspaces are called ad-nilpotent ideals and there are Catalan number of such subspaces. Each ad-nilpotent ideal meets a unique largest nilpotent orbit in the Lie algebra of all matrices. The main result of the paper is that under an equivalence relation on ad-nilpotent ideals studied by Mizuno and others, the equivalence classes are the ad-nilpotent ideals with the same largest nilpotent orbit. We include two applications of the result, one to the higher vanishing of cohomology groups of vector bundles on the flag variety and another to the Kazhdan-Lusztig cells in the affine Weyl group of the symmetric group. Finally, some combinatorial results are discussed.

==> sommers.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amscd}
\usepackage{amsthm}
%\usepackage[francais,english]{babel}

\catcode`\@=11 

%\newcommand{\l@ng}[2]{\iflanguage{francais}{#2}{#1}}
\newcommand{\l@ng}[2]{#1}

\newcommand{\C}{{\mathbb C}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\sln}{{\mathfrak{sl}}}
\newcommand{\gln}{{\mathfrak{gl}}}
\newcommand{\spn}{{\mathfrak{sp}}}
\newcommand{\son}{{\mathfrak{so}}}
\newcommand{\nilcone}{\mathcal{N}}
\newcommand{\orb}{{\mathcal O}}

\newcommand{\DomWeights}{{\Lambda_+}}
\newcommand{\Weights}{\Lambda}
\newcommand{\Roots}{\Delta}
\newcommand{\PosRoots}{{\Delta_+}}
\newcommand{\SimpRoots}{\Pi}
\newcommand{\Sections}{\Gamma}
\newcommand{\irrep}{\widehat}
\newcommand{\Lie}{\mathfrak}

\theoremstyle{plain}
\newtheorem{thm}{\l@ng{Theorem}{Th\'eor\`eme}}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{\l@ng{Lemma}{Lemme}}
\newtheorem{cor}[thm]{\l@ng{Corollary}{Corollaire}}
\newtheorem{clm}[thm]{\l@ng{Claim}{Pr\'etention}}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{des}[thm]{Desideratum}
\newtheorem{thm-}{\l@ng{Theorem}{Th\'eor\`eme}}
\newtheorem{prop-}[thm-]{Proposition}
\newtheorem{lem-}[thm-]{\l@ng{Lemma}{Lemme}}
\newtheorem{cor-}[thm-]{\l@ng{Corollary}{Corollaire}}
\newtheorem{clm-}[thm-]{\l@ng{Claim}{Pr\'etention}}
\newtheorem{conj-}[thm-]{Conjecture}
\newtheorem{des-}[thm-]{Desideratum}

\theoremstyle{definition}
\newtheorem{defn}[thm]{\l@ng{Definition}{D\'efinition}}
\newtheorem{defn-}[thm-]{\l@ng{Definition}{D\'efinition}}
\newtheorem{conv}[thm]{Convention}
\newtheorem{conv-}[thm-]{Convention}
\newtheorem{cond}[thm]{Condition}
\newtheorem{cond-}[thm-]{Condition}

\theoremstyle{remark}
\newtheorem{rmk}[thm]{\l@ng{Remark}{Remarque}}
\newtheorem{exam}[thm]{\l@ng{Example}{Exemple}}
\newtheorem{rmk-}[thm-]{\l@ng{Remark}{Remarque}}
\newtheorem{exam-}[thm-]{\l@ng{Example}{Exemple}}
%\newtheorem*{ppty}{Property}

\renewcommand{\proofname}{\l@ng{Proof}{D\'emonstration}}

\newenvironment{dummy}{}{}

\newcounter{casify}
\newenvironment{casify}%
  {\begin{list}{{\it Case \arabic{casify}}. }
    {\usecounter{casify}
      \setlength{\leftmargin}{0pt}
      \setlength{\rightmargin}{0pt}
      \setlength{\labelwidth}{0pt}
      \setlength{\labelsep}{0pt}
      \setlength{\itemindent}{\parindent}}}
  {\end{list}}

\let\enumdepth\@enumdepth
\newcounter{enumsave}
\newenvironment{enumgen}[1]
  {\setcounter{enumsave}{\enumdepth}
     \enumdepth=#1
     \begin{enumerate}
     \ifnum\enumdepth>1 \renewcommand{\theenumi}{} \fi
     \ifnum\enumdepth>2 \renewcommand{\theenumii}{} \fi
     \ifnum\enumdepth>3 \renewcommand{\theenumiii}{} \fi
     \ifnum\enumdepth>4 \renewcommand{\theenumiv}{} \fi}
  {\end{enumerate} \enumdepth=\theenumsave}

\newcommand{\textx}[1]{\text{\begin{tabular}{c}#1\end{tabular}}}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\gr}{gr}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\real}{Re}
\DeclareMathOperator{\imag}{Im}
\DeclareMathOperator{\vcurl}{curl}
\DeclareMathOperator{\vgrad}{grad}
\DeclareMathOperator{\vdiv}{div}
\DeclareMathOperator{\cmod}{mod}
\DeclareMathOperator{\cHom}{\mathcal{H}\!\mathit{om}}
\DeclareMathOperator{\cExt}{\mathcal{E}\!\mathit{xt}}
\edef\det{\det\nolimits}

\newcommand{\wedgepwr}[1]{\mathchoice%
  {{\textstyle\bigwedge\nolimits^{#1}}}%
  {{\bigwedge^{#1}}}{{\bigwedge^{#1}}}{{\bigwedge^{#1}}}}
\newcommand{\inv}{^{-1}}
\newcommand{\trans}{^{\mathrm t}}
\newcommand{\Langdual}{{^{\scriptscriptstyle L\!}}}
\newcommand{\precheck}{{^{\scriptscriptstyle\vee\!}}}
\newcommand{\postcheck}{^{\scriptscriptstyle\vee}}

\newcommand{\quspace}{\vspace{0.25in}}
\newcommand{\haspace}{\vspace{0.50in}}
\newcommand{\whspace}{\vspace{1.00in}}
\newcommand{\sqspace}{\vspace{1.50in}}
\newcommand{\spacer}{\vspace{0pt plus \baselineskip}}

\catcode`\@=12

